How Large Are Lions? Inducing Distributions over Quantitative Attributes

Most current NLP systems have little knowledge about quantitative attributes of objects and events. We propose an unsupervised method for collecting quantitative information from large amounts of web data, and use it to create a new, very large resource consisting of distributions over physical quantities associated with objects, adjectives, and verbs which we call Distributions over Quantitative (DoQ). This contrasts with recent work in this area which has focused on making only relative comparisons such as "Is a lion bigger than a wolf?". Our evaluation shows that DoQ compares favorably with state of the art results on existing datasets for relative comparisons of nouns and adjectives, and on a new dataset we introduce.

==> tables/FC_new_split_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|rr}
Data        & Dev   & Test \\ \hline
Original Split      & 0.76  & 0.76 \\ \hline
New Split   & 0.70  & 0.71
\end{tabular}
\caption{Accuracy of the Yang et al. model on the original, leaky, split and the new, non-leaky split.}
%These are not entirely comparable, as it's not the same dev/test sets. But if we only drop the training example which cause the bias, a claim might be that we decreased the training size, so obviousely the performance droped. Here in practice the training size is even bigger!
% In practice this is the PCE(LSTM) ensemble model
\label{tbl:new_split_acc}
\end{table}

==> tables/results_clean.tex <==
\begin{table*}[t]
\begin{tabular}{l|llll|llll}
                                 & \multicolumn{4}{l}{Dev}     & \multicolumn{4}{l}{Test}    \\ \hline
Model                            & size & weight & speed & All & size & weight & speed & All \\ \hline
Majority Label                   & 0.51  & 0.64  & 0.74  & 0.54  & 0.53   &  0.68  & 0.78 & 0.57    \\
Forbes \& Choi (Model B)         &  &    &   &     & & &   &     \\
Yang et al (PCE LSTM)            & 0.86 & 0.85   & 0.88  & 0.86  & 0.87   &  0.87  & 0.83   &  0.87   \\ \hline
\rnacronym\                        & 0.82  & 0.75  & 0.51  & 0.78  & 0.81   &  0.77  &  0.35  &  0.77     \\
\rnacronym\ + 10-distance          & 0.81  & 0.76  & 0.51  & 0.78  &  0.81  &  0.77  &  0.34  &  0.77     \\
\rnacronym\ + 3-distance           & 0.84  & 0.78  & 0.58  & 0.81  &  0.84  &  0.80  &  0.42  &  0.80    
\end{tabular}
\caption{Results on the Forbes \& Choi dataset, without the Not-Comparable objects}
\label{tbl:dataset-clean-results}
\end{table*}


==> tables/results_new.tex <==
\begin{table*}[t]
\begin{tabular}{l|llll|llll}
                                 & \multicolumn{4}{l}{Dev}     & \multicolumn{4}{l}{Test}    \\ \hline
Model                            & size & weight & speed & All & size & weight & speed & All \\ \hline
Majority Label                   & 0.55  & 0.48 & 0.50 & 0.51 & 0.48  & 0.44 & 0.53 & 0.50    \\
% Forbes \& Choi (Model B)         &  &    &   &     & & &   &     \\
Yang et al (PCE LSTM)            & 0.56  & 0.61 & 0.64 & 0.60 & 0.58  & 0.53 & 0.60 & 0.57    \\
\rnacronym\                       & 0.63  & 0.62 & 0.58 & 0.61 & 0.62  & 0.59 & 0.65 & 0.62    \\
\rnacronym\ + 10-distance          & 0.64  & 0.62 & 0.58 & 0.62 & 0.62  & 0.58 & 0.65 & 0.62   \\
\rnacronym\ + 3-distance           & 0.65  & 0.64 & 0.58 & 0.63 & 0.63  & 0.59 & 0.62 & 0.61   
\end{tabular}
\caption{Results on the our new created dataset}
\label{tbl:dataset-new-result}
\end{table*}


==> tables/results_original.tex <==
\begin{table*}[t]
\begin{tabular}{l|llll|llll}
                                 & \multicolumn{4}{l}{Dev}     & \multicolumn{4}{l}{Test}    \\ \hline
Model                            & size & weight & speed & All  & size & weight & speed & All \\ \hline
Majority Label                   & 0.50 & 0.54   & 0.53  &      & 0.51 & 0.55   & 0.50  &     \\
Forbes \& Choi (Model B)         & 0.75 & 0.74   & 0.66  &      & 0.75 & 0.76   & 0.72  &     \\
Yang et al (PCE LSTM)            & 0.79 & 0.81   & 0.72  & 0.78 & 0.80 & 0.79   & 0.71  & 0.77 \\
\rnacronym\                        & 0.73 & 0.65   & 0.38  & 0.60 & 0.72 & 0.66   & 0.38  & 0.60 \\
\rnacronym\ + 10-distance          & 0.73  & 0.66  & 0.38  & 0.60 & 0.73 & 0.67   & 0.36  & 0.60   \\
\rnacronym\ + 3-distance           & 0.76  & 0.68  & 0.38  & 0.62 & 0.76 & 0.67   & 0.36  & 0.61   
\end{tabular}
\caption{Results on the Forbes \& Choi dataset, noisy dataset}
% Results with our method is using 15% outlier removal, median as a function, and no data means no value (or zero)
\label{tbl:dataset-noisy-results}
\end{table*}
